Monte Carlo Thought Search: Large Language Model Querying for Complex Scientific Reasoning in Catalyst Design

Discovering novel catalysts requires complex reasoning involving multiple chemical properties and resultant trade-offs, leading to a combinatorial growth in the search space. While large language models (LLM) have demonstrated novel capabilities for chemistry through complex instruction following capabilities and high quality reasoning, a goal-driven combinatorial search using LLMs has not been explored in detail. In this work, we present a Monte Carlo Tree Search-based approach that improves beyond state-of-the-art chain-of-thought prompting variants to augment scientific reasoning. We introduce two new reasoning datasets: 1) a curation of computational chemistry simulations, and 2) diverse questions written by catalysis researchers for reasoning about novel chemical conversion processes. We improve over the best baseline by 25.8\% and find that our approach can augment scientist's reasoning and discovery process with novel insights.

==> emnlp2023-latex/backup/results.tex <==
\section{Experiments}

\begin{table}[tbp]
\centering
\caption{TBD}
\vspace{-0.5em}
    % \resizebox{0.5\textwidth}{!}{ 
\begin{tabular}{p{3.5em}|cc|cc}
    \hline
 &\multicolumn{2}{c|}{\textbf{OpenCatalysis}}&\multicolumn{2}{c|}{\textbf{BioFuels}}\\\hline
Method & Reward & $N_q $& Reward & $N_q$\\\hline\hline
CoT & 2.04 & 2 & 2.23 & 4.\\\hline
Sampling & 3.43 & 20. & 6.41 & 31.\\\hline
ToT & 9.91 & 505.8 & TBD & TBD\\\hline
MCR & 12.47 & 601.8 & 13.77 & 950.5\\\hline\hline
\end{tabular}
% }
\label{tab:multi-relation}
\vspace{-0.5em}
\end{table}

In this section, we present evaluation of $\ourSystem$'s performance across queries representing diversity in chemical reactions as well varying the reasoning complexity.  We also perform a qualitative evaluation of $\ourSystem$'s outputs through rigorous evaluation by researchers specialized in catalysis design.
% \carl{There's a lot of sections here which we probably don't want for a short paper due to space. (each 5.4.1 etc. takes up a line) }

\textbf{Datasets} We conduct our experiments on two catalysis datasets. The first one is curated from the OC20 \cite{chanussot2010open} and OC22 \cite{tran2023open} datasets published by the OpenCatalysis project \cite{zitnick2020introduction}.  The second one is a newly developed dataset with complex reasoning queries focused on biofuels-focused catalyst discovery.  Please see section \ref{sec:datasets} for details on these datasets.  We will release both these datasets upon acceptance of the paper.

\textbf{Baselines} We benchmark $\ourSystem$'s performance with three recent methods: 1) Chain-Of-Thought (CoT) prompting \cite{kojima2022large}, 2) an adaptation of Self-consistency based CoT \cite{wang2022self}, 3) breadth-first-search based Tree-of-Thoughts \cite{yao2023tree}.  
We did not include the depth-first-search method from Tree-of-Thoughts because our search does not have a clear ending criterion.  All our experiments are based on the GPT-3.5 text-davinci-003 model.  Our preliminary evaluations included Galactica \cite{taylor2022galactica} models with 6.7B and 30B parameters.  However, it's responses to chain-of-thought queries with instruction following (to generate list of candidates and then invoking the reward function computation over the returned list) lacked consistency to meet query chaining needs with $\ourSystem$.

% \subsection{Baselines \carl{This should probably be in appendix. We can refer the reader there. Also need to add citations.}}
% We evaluate $\ourSystem$'s performance with the following language models: (can try Galactica \carl{remove this}), GPT-3.5, (also trying GPT-4).
% \begin{enumerate}
%     \item \textsl{Single-Shot Query}: For each of these language models, we execute a query and parse the answer $A$ (such as a recommended catalyst) from the model generated response.  We return a pair ($A$, reward($A$)) as the answer. 
%     \item \textsl{Single-Shot Query with CoT prompt}: For each of these language models, we execute a query and parse the answer $A$ (such as a recommended catalyst) from the model generated response.  We return a pair ($A$, reward($A$)) as the answer. 
%     \item \textsl{Most Frequent Answer}: Given a language model, we execute the same query $N$ times following the above process.  Given this answer set $A_N$, we return a pair ($A_f$, reward($A_f$)) as the answer, where $A_f$ is the most frequently occurring answer in $A_N$.
%     \item \textsl{Most Frequent Answer with CoT prompt}: Given a language model, we execute the same query $N$ times following above process.  Given this answer set $A_N$, we return a pair ($A_f$, reward($A_f$)) as the answer, where $A_f$ is the most frequently occurring answer in $A_N$.
%     \item Comparison with BFS and DFS implementation (used in the Tree-of-Thought paper).
% \end{enumerate}

% \subsection{Metrics \carl{Probably want most of this in the appendix, although I'm not sure we are using these metrics anymore anyway?}}
% \textbf{Reward ratio}: Given a query $Q$, reward function $f_R(\cdot)$ we compare the rewards across a baseline method $M$ and $\ourSystem$ by computing the ratio $f_R(MCR(Q))/f_R(M(Q))$.

% \begin{table}
%     \centering
%     \caption{Caption for table \carl{Add column for # acerage API calls. Possibly column with results for OpenCatalysis}}
%     {\begin{tabular}{ccc}
%     &\bf{OpenCatalysis} & \bf{BioFuels}\\
%     Single Shot&2.04&2.23\\
%     Multi Shot&3.43&6.410833\\
%     BFS&9.91&\\
%     MCR&12.47&13.765
%     \end{tabular}}
%     \label{tab:settings}
% \end{table}





% \begin{table}
%     \centering
%     \caption{Caption for table \carl{Add column for # acerage API calls. Possibly column with results for OpenCatalysis}}
%     {\begin{tabular}{ccc}
%     &\bf{OpenCatalysis} & \bf{BioFuels}\\
%     Single Shot&2.04&2.23\\
%     Multi Shot&3.43&6.410833\\
%     BFS&9.91&\\
%     MCR&12.47&13.765
%     \end{tabular}}
%     \label{tab:settings}
% \end{table}

% \textbf{Precision and MRR}: Alternatively, if the domain experts provide us with a correct or preferred answer for each query AND if we could retrieve a list from all querying methods then we can also compute the precision/recall and mean reciprocal rank (MRR).  

% Precision = Number of queries in which a query answer contains correct answer/Number of Queries

% If our method/all methods return a list, then MRR would capture where the correct answer falls in the list.  Methods that rank the correct answer higher in its answer list would get a higher score.

\heng{define reward function formally}



\subsection{Qualitative Analysis Against Expert Reasoning}

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.48\textwidth]{emnlp2023-latex/figures/eval-tree-depth-cost.png}
\caption{Illustration of an evaluation by a domain expert on the progression of top search results found on the path to the answer with highest reward.}
\label{fig:eval-1-mcr}
\end{figure}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/eval-1-qa.png}
\caption{Example question and human answer from our compiled QA-dataset.}
\label{fig:eval-1-qa}
\end{figure*}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/eval-1-gpt-3.5.png}
\caption{Response to above query returned by GPT-3.5.}
\label{fig:eval-1-gpt-3}
\end{figure*}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/eval-1-mcr.png}
\caption{Response to above query returned by MCR.}
\label{fig:eval-1-mcr}
\end{figure*}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.5\textwidth]{emnlp2023-latex/figures/eval-1-comp.png}
\caption{Comparison of MCR vs GPT-3.5 by domain expert.}
\label{fig:eval-1-mcr}
\end{figure*}



\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.6\textwidth]{emnlp2023-latex/figures/eval-tree-depth-no-cost.png}
\caption{Illustration of an evaluation by a domain expert on the progression of top search results found on the path to the answer with highest reward.}
\label{fig:eval-1-mcr}
\end{figure*}

\textcolor{blue}{Henry} Get output for 5 queries from the catalysis dataset (mcr, singleshot, singleshot frequent, bfs)

\textcolor{blue}{Sutanay} Compare answers with expert answer




==> emnlp2023-latex/new-introduction.tex <==

\section{Introduction}

% For example, finding the optimal combination of functional groups is at the core of multi-objective optimization for drug design \cite{you2018graph, ward2021benchmarking}.  
\iffalse
Many exploratory queries for scientific research and discovery are characterized by attempts to find optimal combinations of factors that maximizes a property of interest \carl{This is good but could be ``catchier'' maybe? Can we rephrase to start the sentence with "Scientific Discovery"?}.  Given a chemical reaction, finding the optimal combination of operating conditions--reactants (the reaction's input), environmental conditions (e.g. temperature), and catalysts (substances that increase the reaction rate)--is essential to discovering new energy-efficient fuels \cite{yang2019machine, tran2023open, zitnick2020introduction} or lower-energy chemical conversion processes (Fig. \ref{fig:challenge_and_approach}). For highly empirical scientific fields such as chemistry, such combinatorial searches coupled with scientific reasoning is performed by practitioners for hypothesis generation and testing.  The emerging capability of large language models (LLMs) to reason in human-comprehensible terms \cite{wei2022chain, ouyang2022training, taylor2022galactica, BiomedicalLM2023, openai2023gpt4} provides an opportunity to accelerate the cycle of scientific discovery via autonomous machine reasoning.  
\fi
% Most scientific discoveries rely on the logical sifting of optimal combinations of factors that maximize a property of interest. %
% Uncovering the optimal combinations of factors that maximize a property of interest is of critical importance for scientific  discovery in many fields. 
Scientific discovery thrives on understanding which combinations of factors influence a property of interest. With a robust enough understanding of these factors, one can optimize the property of interest through a combinatorial optimization process. In some cases, such a search can be automated through a Bayesian Optimization process (https://pubs.rsc.org/en/content/articlelanding/2021/me/d1me00093d).
For highly empirical fields such as catalysis, such combinatorial searches require complex scientific reasoning, which is mentally performed by practitioners for hypothesis generation. For example, to discover new energy efficient fuels \cite{yang2019machine, tran2023open, zitnick2020introduction} or efficient chemical conversion processes requiring less energy, a scientist would need to consider the chemical reaction, the reactants that undergo the reaction, the catalysts that improve the rate of reaction, and find the optimal combination of operating conditions (Fig. \ref{fig:challenge_and_approach}). An wide understanding of the scientific literature is required to navigate such a search space.
The emerging capability of knowledge-aware large language models (LLMs) \cite{wei2022chain, ouyang2022training, taylor2022galactica, BiomedicalLM2023, openai2023gpt4} provides an opportunity to augment scientists' reasoning to accelerate the cycle of scientific discovery via autonomous machine reasoning.

\begin{figure*}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/challenge_and_approach.png}
\caption{Illustration of the combinatorial thinking used by human experts to reason about a catalyst (best viewed in color).  They successively ``think in terms of" different constraints and factors, each of which are related via scientific principles, and narrow down the set of possible candidates.  Our Monte Carlo Reasoner emulates such cognitive thinking by prompting a language model with different combinations, yielding a tree-structured space of queries and potential candidates, and returns the optimal answer via efficient exploration of the possible space.  }
\label{fig:challenge_and_approach}
\end{figure*}

Despite their promise, the sensitivity of language models to their inputs and hallucination remain areas for concern \cite{creswell2022faithful, taylor2022galactica}. In addition to addressing these challenges, providing answers with high specificity using key technical terminology (Fig. \ref{fig:challenge_and_approach}) is essential to earn the scientific community's trust and pave the way for adoption of machine reasoning systems. 

In this work, we focus on the problem of suggesting the top-$k$ catalysts for a given chemical reaction and generating the reasoning for each candidate. In collaboration with researchers from the catalysis community, we developed a new dataset, BioFuels Question Reasoning (\dataset), of complex reasoning questions and answers.  We observe the reasoning pathways used by domain scientists and conclude that it is important for LLMs to progress from ``thinking step-by-step'' to ``thinking step-by-step in terms of relevant properties''. In this setting, we are given a question which has relevant chemical properties $\mathbf{P},|\mathbf{P}|=n$ (e.g. \{``crystal planes'', ``toxicity''\}) and we want to identify the best subset $\mathbf{R\subset \mathbf{P}},|\mathbf{R}|=r$ for the language model to ``think'' in terms of. Considering that language models are sensitive to input permutations, there are $P^{n}_{r}=\frac{n!}{(n-r)!}$ possible prompts. This goal can be accomplished by learning to prompt the LLM with the most relevant subset of properties \cite{deng-etal-2022-rlprompt} or decomposing the set into a sequence of chained queries \cite{dohan2022language}. In both cases, identification of the prompt-generating property subset becomes the limiting factor. 

 To solve this problem, we propose \underline{M}onte \underline{C}arlo \underline{R}easoner ($\ourSystem$), a generic methodology that addresses the combinatorial challenge of query decomposition. Considering the practical challenges of learning prompts that are both human comprehensible (a key consideration for scientists) and provide the best performance \cite{deng-etal-2022-rlprompt}, we pursue a stochastic, heuristic search-based approach that leverages LLMs trained on scientific literature with sophisticated instruction following capabilities \cite{ouyang2022training}.
 
 We formulate the task as a search problem in which an agent performs a query in an uncertain environment (represented by the LLM) and determines a query variant to pursue based on the perceived reward. Given an initial query, we construct a tree structure of these unique query variants in order to progressively refine the original query (the root) into property-specific variations (the leaves).  We use a Monte Carlo Tree Search algorithm (MCTS) to perform stochastic search over this space of possible queries. %Each node in the tree represents an unique query and an estimation of its reward. 
 
 % \heng{define reward, and what it's used for} 

%Our second major contribution in this paper comes from demonstrating the value of a scientific domain-specific reward function into LLM-based computations.  Estimation of the energy of a chemical structure is at the core of developing efficient chemical reactions (see section \ref{sec:motivation_energy_func} for details).  Finding catalysts that can enable chemical reactions with least amount of external energy is key to developing environmentally friendly industrial processes. In this work, we implement such energy function specific considerations via a LLM-derived reward function.  Our experiments (using questions detailed in Table \ref{fig:qa_table_biofuels}) show that a simplistic integration of such a fundamental scientific concept dramatically improves the specificity of answers and their associated reasoning from the LLM.
Our second major contribution is demonstrating the efficacy of using a scientific domain-specific reward function in LLM-based computations.  Estimation of the energy of a chemical structure is at the core of developing efficient chemical reactions (see Appendix \ref{sec:motivation_energy_func} for details).  Finding catalysts that can enable chemical reactions with the least amount of external energy is key to developing environmentally friendly industrial processes. In this work, we implement such energy function specific considerations via a LLM-derived reward function. Our experiments (using questions detailed in Table \ref{fig:qa_table_biofuels}) show that even a simplistic reward function dramatically improves the specificity of answers and their associated reasoning from the LLM. 

\noindent In summary, we make the following contributions:
\begin{enumerate}[leftmargin=*]
\itemsep-0.3em 
    \item We present \textsl{Monte Carlo Reasoner (MCR)}, an algorithm to prompt LLMs for zero-shot complex reasoning tasks involving combinatorial search.
    % prompt strategy generation for LLM-driven complex scientific reasoning tasks as a stochastic search problem in an uncertain environment and propose a Monte Carlo Tree Search-based approach.
    \item We introduce a new chemistry-focused dataset, \dataset, that captures key reasoning challenges in hypothesis generation and testing faced daily by scientists. We present in-depth qualitative analysis of $\ourSystem$ on \dataset.
    \item We demonstrate that a domain-specific reward function that represents a fundamental scientific concept can lead to dramatic improvement in the quality and specificity of LLM answers.
    % \item We demonstrated the impact of our methodology towards LLM-driven hypothesis generation for the chemistry domain, especially focusing on the discovery of new catalysts for energy efficient chemical reactions.
    % \item We developed a new dataset that builds upon previous efforts from the computational chemistry community and introduce new LLM-based reasoning tasks.

\end{enumerate}

% \textcolor{red}{In contribution: ``we perform in-depth qualitative analysis from expert researchers in a scientific field with a high barrier for analysis.'' needs rewording}
 
  % focus on finding novel Given each query and its answers, we execute a reward function to rank potential answers.  For example, given a target chemical compound, the amount of external energy expended for its production is a measure of its desirability and of the process used to produce it.  Such measures can be computed by a language model either through a prompt or via delegation to an external function.  Assuming the reward surface is smooth as we construct and navigate the tree, our stochastic tree search systematically explores the query space and returns the best possible answer.

% Returning to our focus into chemistry-specific challenges, answering a question such as finding top-K catalysts for a given reaction and specific conditions requires reasoning about different factors. Additionally, for such answers to drive scientific hypothesis generation and inspire further consideration, scientists prefer answers that are grounded in specific technical concepts over simplified answers that could gleaned from general purpose resources such as Wikipedia (see Fig. TBD).  In terms of querying a LLM, such results can be achieved either through prompting the LLM with most relevant subset of scientific concepts, or decomposing the set into a sequence of chained-queries \cite{dohan2022language}.  In either way, identification of the prompt-generating subset becomes the limiting factor.  





% We formally define such queries as follows: 1) an initial specification of the problem (hereby described as a ``base query”) and 2) ``actions” that further constrain the query, and 3) an evaluation function that ranks candidate answers.   We posit that the language model can implicitly make the logical associations between the specified constraints and does not require explicit specification such as a database or knowledge graph query.  

% Our work is motivated by prior research that demonstrates that the most efficient prompts may not be human readable.  Therefore, seeking to generate most human-interpretable queries may further require alignment between logical representation of a scientific domain and the language model’s internal representation of said knowledge.   




% The sensitivity of language models to their input has triggered much research on learning and designing effective prompts \cite{deng-etal-2022-rlprompt}.  Approaches such as chain-of-thought (CoT) prompting \cite{kojima2022large} have became popular for generating responses with reasoning, especially for models trained with human feedback.  Much of the research in this area has focused on arithmetic reasoning, in which a mathematical task is solved in a step-by-step fashion~\cite{wei2022chain, reversecot2023}.  Given a specific task, reinforcement learning with human feedback (RLHF) methods and CoT variants \cite{zelikman2022star} collectively focus on improving the answer accuracy as well as reasoning.  The methods demonstrate that prompts that invoke reasoning not only improve the explainability of the language model output, but also lead to improvement in the answer accuracy itself.  Going beyond RLHF and CoT methods, it has also been shown that decomposition of a complex question into a sequence of tasks, or query decomposition, leads to further improvement in model performance \cite{creswell2022faithful, creswell2022selection, dohan2022language, jung2022maieutic, zhou2022least, wang2022self, yao2023tree}.

% \heng{elaborate why this is a challenging problem? how big is the search space? and why LLMs can help?}
% \heng{here needs a transition sentence, say we are using XXX problem in the chemical area as a case study.}
% \sutanay{Leaving Heng's questions to see how they have been addressed.}





  % Another related topic in this context is the non-deterministic aspect of querying language models.  The same question posed to the language model can elicit different answers and the variations increase with the complexity and size of query context.  If the environment is stochastic there is an inevitable uncertainty in the model’s predictions.







% Many scientific fields such as chemistry are highly empirical.  For example, discovering new catalysts is key to breakthroughs in designing the energy efficient chemical processes, and in past such discovery has largely followed an experiment-driven path.  Many scientific fields such as catalysis do not have a massive amount of observational data, which has limited potential for big data-driven machine-learning tools.  For them selective experiment design is crucial for minimizing costs and delays to key results.  However, experiment design is an art that strongly depends on a researcher’s knowledge of the extensive literature and ability to reason about promising hypotheses.  Large language models trained from scientific literature can be particularly impactful for such ideation and hypothesis generation.  In this work, we focus on the catalyst recommendation problem: given a set of reactants, an initial candidate catalyst and operating conditions such as pressure and temperature, what are the most optimal catalysts to recommend? 



% For example, Figure 1a shows an example response from GPT-3.5. However, we can execute the same query repeatedly with varied random seeds and obtain different answers.  Figure 1b shows a distribution of candidate catalysts from $N$-execution of the query.  In short, this illustrates a class of reasoning queries where we need to explore the space of possible queries and answers, and produce a list of ranked candidates, each accompanied by different ``chain-of-thoughts".  Finally, Figure 1c shows how this query space can be explored via two dimensions.  We can generate specialized queries and progressively generate narrower candidate spaces by considering more scientific concepts.  Given a set of scientific concepts, we can also generate multiple query variants with different semantic interpretations. \heng{here need to define what are queries and answers}

